Capturing the temporal constraints of gradual patterns

Gradual pattern mining allows for extraction of attribute correlations through gradual rules such as: "the more X, the more Y". Such correlations are useful in identifying and isolating relationships among the attributes that may not be obvious through quick scans on a data set. For instance, a researcher may apply gradual pattern mining to determine which attributes of a data set exhibit unfamiliar correlations in order to isolate them for deeper exploration or analysis. In this work, we propose an ant colony optimization technique which uses a popular probabilistic approach that mimics the behavior biological ants as they search for the shortest path to find food in order to solve combinatorial problems. In our second contribution, we extend an existing gradual pattern mining technique to allow for extraction of gradual patterns together with an approximated temporal lag between the affected gradual item sets. Such a pattern is referred to as a fuzzy-temporal gradual pattern and it may take the form: "the more X, the more Y, almost 3 months later". In our third contribution, we propose a data crossing model that allows for integration of mostly gradual pattern mining algorithm implementations into a Cloud platform. This contribution is motivated by the proliferation of IoT applications in almost every area of our society and this comes with provision of large-scale time-series data from different sources.

==> frontmatter/nomenclature.tex <==
%---------------------------------------------------------
%	NOMENCLATURE
%---------------------------------------------------------

%\addcontentsline{toc}{chapter}{Abbreviations}
\cleardoublepage \phantomsection
\mtcaddchapter[Nomenclature]

	\nomenclature{$\varrho$}{User-specified minimum support of frequent pattern}
	\nomenclature{$\delta$}{User-specified minimum representativity of frequent pattern}
	\nomenclature{$\sigma$}{Rank of an object}
 
	\printnomenclature
	

==> frontmatter/quote.tex <==

%----------------------------------------------------
%	QUOTATION PAGE
%----------------------------------------------------

\vspace*{0.2\textheight}
\bigbreak
\bigbreak
\rightline{\textit{``If I have seen further it is by standing on the shoulders of Giants''}}
\hfill Sir Isaac Newton (1642 – 1727)


